Matching Algorithms in the Sparse Stochastic Block Model

The stochastic block model (SBM) is a generalization of the Erd\H{o}s--R\'enyi model of random graphs that describes the interaction of a finite number of distinct communities. In sparse Erd\H{o}s--R\'enyi graphs, it is known that a linear-time algorithm of Karp and Sipser achieves near-optimal matching sizes asymptotically almost surely, giving a law-of-large numbers for the matching sizes of such graphs in terms of solutions to an ODE. We provide an extension of this analysis, identifying broad ranges of stochastic block model parameters for which the Karp--Sipser algorithm achieves near-optimal matching sizes, but demonstrating that it cannot perform optimally on general SBM instances. We also consider the problem of constructing a matching online, in which the vertices of one half of a bipartite stochastic block model arrive one-at-a-time, and must be matched as they arrive. We show that the competitive ratio lower bound of 0.837 found by Mastin and Jaillet for the Erd\H{o}s--R\'enyi case is tight whenever the expected degrees in all communities are equal. We propose several linear-time algorithms for online matching in the general stochastic block model, but prove that despite very good experimental performance, none of these achieve online asymptotic optimality.

==> cmds.tex <==
% COMMANDS AND HOTKEYS 
%\mathbb commands.
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\J}{\mathbb{J}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\usepackage{bbm}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\0}{\mathbbm{0}}

%\mathcal commands.
\newcommand{\A}{\mathcal{A}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Cs}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\K}{\mathcal{K}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\ps}{\mathcal{P}}
\newcommand{\Rc}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\hbt}{\frac{\hbar}{2}}

%text shortcuts.
\newcommand{\dne}{\text{ DNE}}
\newcommand{\und}{\text{ undefined}}
\newcommand{\ad}{\text{ and }}
\newcommand{\fs}{\text{ for some }}
\newcommand{\we}{\text{ where }}
\newcommand{\wee}{\text{ where:}}
\newcommand{\st}{\text{ such that }}
\newcommand{\stt}{\text{ such that:}}
\newcommand{\wh}{\text{ we have }}
\newcommand{\wht}{\text{ we have that }}
\newcommand{\wi}{\text{ with }}
\newcommand{\el}{Euler-Lagrange Equation }
\newcommand{\eln}{Euler-Lagrange Equation}
\newcommand{\els}{Euler-Lagrange Equations }
\newcommand{\elsn}{Euler-Lagrange Equations}
\newcommand{\he}{Hamilton Equation }
\newcommand{\hen}{Hamilton Equation}
\newcommand{\hes}{Hamilton Equations }
\newcommand{\hesn}{Hamilton Equations}
\newcommand{\hje}{Hamilton-Jacobi Equation }
\newcommand{\hjen}{Hamilton-Jacobi Equation}
\newcommand{\sa}{$\sigma$-algebra }
\newcommand{\san}{$\sigma$-algebra}

%math single character shortcuts.
\newcommand{\fa}{\forall}
\newcommand{\eq}{\exists}
\newcommand{\imp}{\implies}
\newcommand{\dnimp}{\centernot\implies}
\newcommand{\cd}{\cdot}
\newcommand{\ceq}{\coloneqq} % :=
\newcommand{\sbs}{\subseteq}
\newcommand{\sps}{\supseteq}
\newcommand{\nsbs}{\not\subseteq}
\newcommand{\nsps}{\not\supseteq}
\newcommand{\nin}{\notin}
\newcommand{\sqsbs}{\sqsubseteq} % square subseteq

%math shortcut commands.
\newcommand{\Bp}{\B^\ast}
\newcommand{\f}{f^{-1}}
\newcommand{\e}{\varepsilon}
\newcommand{\de}{\delta}
\newcommand{\es}{\varnothing}
% \newcommand{\lp}{\ell^p}
\newcommand{\sm}{\setminus}
\newcommand{\p}{\partial}
\newcommand{\pr}{\, '}
% \newcommand{\indep}{\ensuremath{\! \! \perp \! \! \! \perp \!}}
\newcommand{\vf}{\vec{F}}
\newcommand{\vtau}{\vec{\tau}}
\newcommand{\vnab}{\vec{\nabla}} %vector gradient
\newcommand{\dotp}{\dot{\mathcal{P}}}
\newcommand{\dotq}{\dot{\mathcal{Q}}}
% \newcommand{\norm}{\| \circ \|}
\newcommand{\Co}{ \Cs \left( 0,1 \right) }
\newcommand{\Ca}{ \Cs \left( a,b \right) }
\newcommand{\FF}{ \{ F_\alpha \}_{\alpha \in I}}
\newcommand{\GG}{ \{ G_\alpha \}_{\alpha \in I}}
\newcommand{\HH}{ \{ H_\alpha \}_{\alpha \in I}}
\newcommand{\KK}{ \{ K_\alpha \}_{\alpha \in I}}
\newcommand{\Ro}{ \mathcal{R} \left( \left[ 0,1 \right] \right) }
\newcommand{\Ra}{ \mathcal{R} \left( \left[ a,b \right] \right) }
\newcommand{\UU}{ \{ U_\alpha \}_{\alpha \in I}}
\newcommand{\Vp}{\V^\ast}
\newcommand{\QC}{\R \sm \Q}
\newcommand{\Sigmast}{\Sigma^\ast}
\newcommand{\deast}{\de^\ast}
\newcommand{\De}{\Delta}
\newcommand{\Deast}{\De^{\hspace{-0.15 em}\ast}}
\newcommand{\Fhat}{\hat{F}}

% paired delimiters: 
\DeclarePairedDelimiter\absd{\lvert}{\rvert} % absolute val
\DeclarePairedDelimiter\normd{\lVert}{\rVert} % norm
\newcommand{\expectauto}[1]{\E\left[#1\right]} % expectation: auto adjusting
\newcommand{\cov}[1]{\operatorname{Cov}\left[#1\right]}
\newcommand{\corr}[1]{\operatorname{Corr}\left[#1\right]}

% automatic \left\right brackets 
\newcommand{\bpar}[1]{\left(#1\right)}
\newcommand{\bbr}[1]{\left[#1\right]}
\newcommand{\bcurly}[1]{\left\{#1\right\}}

% sums 
\newcommand{\sumlimin}{\sum_{i=1}^n}
\newcommand{\sumlimkn}{\sum_{k=1}^n}
\newcommand{\sumlimizn}{\sum_{i=0}^n}
\newcommand{\sumlimkzn}{\sum_{k=0}^n}
\newcommand{\sumlimyzinf}{\sum_{y=0}^\infty}
\newcommand{\sumlimyoinf}{\sum_{y=1}^\infty}
\newcommand{\sumlimiinf}{\sum_{i=-\infty}^\infty}
\newcommand{\intinfinf}{\int_{-\infty}^\infty }
\newcommand{\sumlimiN}{\sum_{i=1}^N}

%command shortcuts.
\newcommand{\ds}{\displaystyle}
\newcommand{\no}{\noindent}
\newcommand{\vs}{\vspace*}
\newcommand{\hs}{\hspace}
\newcommand{\bs}{\baselineskip}

% math operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\;max}

% probability things
% P(A | B) (given)
\newcommand\given[1][]{\:#1\vert\:}
\newcommand{\Bin}{\mathrm{Bin}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\ind}[1]{\1_{[#1]}} % indicator 
\newcommand{\bigind}[1]{\1_{\left[#1\right]}}  % big indicator
\newcommand{\disteq}{\stackrel{\L}{=}} % distributional equals

% hats and tildes 
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\itilde}{\Tilde{\imath}}


